Tusqh: Topological Control of Volume-Fraction Meshes Near Small Features and Dirty Geometry

This work develops a framework to create meshes with user-specified homology from potentially dirty geometry by coupling background grids, persistent homology, and a generalization of volume fractions. For a mesh with fixed grid size, the topology of the output mesh changes predictably and monotonically as its volume-fraction threshold decreases. Topological anti-aliasing methods are introduced to resolve pinch points and disconnected regions that are artifacts of user choice of grid size and orientation, making the output meshes suitable for downstream processes including analysis. The methodology is demonstrated on geographical, mechanical, and graphics models in 2D and 3D using a custom-made software called Tusqh. The work demonstrates that the proposed framework is viable for generating meshes on topologically invalid geometries and for automatic defeaturing of small geometric artifacts. Finally, the work shows that although subdividing the background grid frequently improves the topological and geometrical fidelity of the output mesh, there are simple 2D examples for which the topology does not converge under refinement for volume-fraction codes.

==> figure_10.tex <==
Figure 10

==> figure_5.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{figure_5.png}
\caption{Volume Fraction: 100\%; $\beta_0 = $(0th Betti number/H0 number); $\beta_1 = $(1st Betti number/H1 number).}
\end{figure}

==> figure_6.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{figure_6.png}
\caption{Volume Fraction: 50\%; $\beta_0 = $(0th Betti number/H0 number); $\beta_1 = $(1st Betti number/H1 number).}
\end{figure}

==> figure_8.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{30x30_Volume_Fraction_Error_Mesh_Winding_Number_vol_0.5.png}
\caption{Volume Fraction: 50\%; $\beta_0 = $2; $\beta_1 = $4.}
\end{figure}

==> figure_9.tex <==
\begin{figure}
\includegraphics[width=\columnwidth]{30x30_Volume_Fraction_Error_Mesh_Winding_Number_vol_0.15.png}
\caption{Volume Fraction: 15\%; $\beta_0 = $1; $\beta_1 = $7. At this low volume fraction threshold the mesh begins to exit the disjoint boundary.}
\end{figure}

==> to_do.tex <==
{\Rd
Let's {\KS make blue} the things that non-Brians can do.
\begin{enumerate}
\item {\KS pinch and archipelago discussion in Conclusion. Other conclusion edits.}
\item 3D smooth example, cowboy (not bunny), PH, betti 2 component; geometry fitting using sculpt for cowboy, or bunny. If doesn't work, then move to future work.
\item copyright software, BYU and Sandia, put on github, drivers for reproducing some of the results, mention reproducibility. status : scott has contacted Sandia copyright.
\item Obtain permission for use of figures 4 and 6 of Generalized Winding Number paper from ACM
\item Make Figure 22 bigger so the text is more readable
\item Fix one of the footnotes in the Results section---could fix using tinyurl
\item Potentially make a 3D figure for primal-dual-simplex conversion to Aleph
\item Upload the document with the appendix of the proof to arXiv on October 14.
\end{enumerate}
}


